When Crowd Meets Persona: Creating a Large-Scale Open-Domain Persona Dialogue Corpus

Building a natural language dataset requires caution since word semantics is vulnerable to subtle text change or the definition of the annotated concept. Such a tendency can be seen in generative tasks like question-answering and dialogue generation and also in tasks that create a categorization-based corpus, like topic classification or sentiment analysis. Open-domain conversations involve two or more crowdworkers freely conversing about any topic, and collecting such data is particularly difficult for two reasons: 1) the dataset should be ``crafted" rather than ``obtained" due to privacy concerns, and 2) paid creation of such dialogues may differ from how crowdworkers behave in real-world settings. In this study, we tackle these issues when creating a large-scale open-domain persona dialogue corpus, where persona implies that the conversation is performed by several actors with a fixed persona and user-side workers from an unspecified crowd.

==> formula.tex <==
For attributes with two label candidates (strange, uneasy, engage, active), the final label is determined by majority voting of three annotators. However, for attributes with three or more label candidates (self, empathy), the final label may not be determined by majority voting, particularly when three annotators make different tagging. In this case, we provide an automatic logic for the final decision.

Let the attribute of interest be $Y$ and each candidate be $y_1, ..., y_C$ where $C$ is the number of label candidates.

For the given dialogue $D = \{d_1, d_2, ... d_K\}$ where $d_k$ denotes each utterance, we first define a set of utterances $U \subseteq [1,K]$ where $U$ is defined as a set of indices $k$ where the final label of $d_k$ is determined based on majority voting. Let $a_1, ..., a_N$ be annotators who tagged the dialogue, and let $F_k (a_n)$ be the label that annotator $a_n$ tagged for the utterance $d_k$. Especially for $k \in U$, let $F_k$ be the pre-defined final label assigned to $d_k$ (which is distinguished from the label determined along with this process).

First, we can make up an $N$-dimensional `reliability matrix' $R$ which is defined as follows:

\begin{equation}
    R_n = (\sum_{k \in U} 1(F_k (a_n) = F_k))/|U|
\end{equation}


where $1$ is the indicator function and $|\cdot|$ denotes the size of the set. However, $R$ does not reveal how each annotator has performed regarding each label candidate. Thus, we make up a $C \times N$ matrix $Q$ which is defined as follows:

\begin{equation}
    Q_{cn} = \frac{\sum_{k \in U} 1(F_k (a_n) = y_c)}{|\{k|k \in U, F_k = y_c\}| }
\end{equation}

We call $Q$ a `modified reliability matrix'. Note that $0$ should be assigned for $Q_{cn}$ if $|\{k|k \in U, F_k = y_c\}| = 0$. 

%% added
We also note that $Q$ reveals how often the annotator detected the majority label but does not reflect how s/he behaves when s/he did NOT belong to the majority. Thus, we make up another $C \times N$ matrix $P$ which is defined as follows:

\begin{equation}
    P_{cn} = \frac{\sum_{k \in U} 1(F_k (a_n) \neq y_c) \cdot 1(F_k (a_n) \neq F_k)}{\sum_{k \in U} 1(F_k (a_n) \neq F_k)}
\end{equation}

We call $P$ an `unreliability matrix'. Note that $0$ should be assigned for $P_{cn}$ if $\sum_{k \in U} 1(F_k (a_n) \neq F_k) = 0$. 
%% added

Now, let $d_l$ be an utterance where the conflict occurred; that is, in the three-annotator environment, $F_l (a_1) \neq F_l (a_2)$, $F_l (a_2) \neq F_l (a_3)$, and $F_l (a_3) \neq F_l (a_1)$. The step for the final decision of the label is as follows:

\begin{itemize}
    \item Considering all the tags $F_l (a_n)$ from the annotators, let's compare the reliability of each tag by making up an $N$-dimensional array $T$ where the $T_n = Q_{F_l (a_n),n} \cdot P_{F_l (a_n),n}$. 
    \item Assign $F_l = F_l(a_t)$ for $t = \texttt{argmax} (T)$, if there is no tie score in $T$.
    \item If tie occurs, assign $F_l = F_l(a_r)$ for $r = \texttt{argmax} (R)$, if there is no tie score in $R$.
    \item If tie occurs again, assign $F_l$ a random candidate between $F_l (a_n)$.
\end{itemize}
